Hidden Markov Model Identifiability via Tensors

The prevalence of hidden Markov models (HMMs) in various applications of statistical signal processing and communications is a testament to the power and flexibility of the model. In this paper, we link the identifiability problem with tensor decomposition, in particular, the Canonical Polyadic decomposition. Using recent results in deriving uniqueness conditions for tensor decomposition, we are able to provide a necessary and sufficient condition for the identification of the parameters of discrete time finite alphabet HMMs. This result resolves a long standing open problem regarding the derivation of a necessary and sufficient condition for uniquely identifying an HMM. We then further extend recent preliminary work on the identification of HMMs with multiple observers by deriving necessary and sufficient conditions for identifiability in this setting.

==> application.tex <==
\section{Application}
\label{sec:application}

In this section, we apply our findings to a problem in anomaly detection on networks. We show how multiple observers can 
turn an unidentifiable HMM in the single observer setting into an identifiable one.

\subsection{Collaborative anomaly detection}

We apply our findings to a problem considered by Nguyen et al.~\cite{Nguyen12MultiHMM,Nguyen12PPHMM}, where 
multiple Internet Service Providers (ISPs) are monitoring the same distributed attack, launched by the an adversary, on their 
own respective networks. The paper \cite{Nguyen12PPHMM} developed privacy preserving protocols to enable ISPs to 
combine their observations and infer the HMM. These practical implementation details are beyond the scope of our paper, 
as we only focus on the identifiability aspect of the problem.

Let there be $m$ ISPs, or equivalently, observers. A Secure Shell (SSH) attack is typically modelled by $q=7$ states 
\cite{Sperotto09SSH}. We set $\bA$ equal to an example constructed from real data \cite{Sperotto09SSH}, presented in equation 
\eqref{eq:transition_SSH}. In this example, $\krank(\bA) = 7$. Each observer $j$ has a level of measurement error $0 \le \epsilon_j 
\le 1$, with the observation matrix given in equation \eqref{eq:observation_SSH}.
\begin{figure*}[t!]
\normalsize
\setcounter{tempcnt}{\value{equation}}
%\addtocounter{tempcnt}{-1}
\setcounter{equation}{\value{tempcnt}}
\be
\bA =
\begin{bmatrix}
0.6170   & 0.3780   & 0.0040   &      0   &      0   &      0   & 0.0010\\
0.1860   & 0.8130   & 0.0010   &      0   &      0   &      0   &      0\\
     0   &      0   & 0.7230   & 0.2350   & 0.0400   &      0   & 0.0010\\
     0   &      0   & 0.2140   & 0.7570   & 0.0290   &      0   &      0\\
     0   &      0   &      0   & 0.0220   & 0.6670   & 0.2670   & 0.0030\\
     0   &      0   &      0   &      0   & 0.1520   & 0.8480   &      0\\
     0   &      0   &      0   &      0   &      0   &      0   & 1.0000
\end{bmatrix}
\label{eq:transition_SSH}
\ee
\vspace{4pt}
\be
\bB^{(j)} = 
\begin{bmatrix}
\epsilon_j & 1-2\epsilon_j & \epsilon_j & 1-2\epsilon_j  &\epsilon_j & 1-2\epsilon_j & 1-2\epsilon_j\\
1-2\epsilon_j & \epsilon_j & \epsilon_j & \epsilon_j  & 1-2\epsilon_j &\epsilon_j & \epsilon_j\\
\epsilon_j & \epsilon_j & 1-2\epsilon_j & 1-2\epsilon_j  &\epsilon_j &\epsilon_j & \epsilon_j
\end{bmatrix}^\T
\label{eq:observation_SSH}
\ee
\hrulefill
\vspace*{4pt}
\end{figure*}

In the homogeneous setting, $\epsilon_j := \epsilon$ for all $j = 1,2,\cdots,m$. Beginning from an initial state $\bpi$ drawn 
from a stationary distribution, let the HMM be parameterised by $\blambdam = \{\bpi; q, \{\kappa_j\}_{j=1}^m, \bA,
\{\bB^{(j)}\}_{j=1}^m \}$ for multiple observers. Here, both $q$ and $\kappa_j,\,\forall j$ are known. The goal is to identify
$\blambdam$ from the observations of multiple observers. For any single observer, the parameter set is $\blambda^{(j)} =
\{\bpi; q, \kappa_j, \bA, \bB^{(j)}\}$.

Consider a single observer $j$. The chief reason why the parameter set $\blambda^{(j)}$ is unidentifiable is the following: 
for any value of $\epsilon_j$, $\krank(\bB^{(j)}) = 1$, since there are at least two rows of $\bB^{(j)}$ that are equal. Since it is 
implied by Theorem \ref{thm:unique_identifiability}, for a single observer, the condition $\krank(\bB^{(j)}) \ge 2$ must hold, there is 
no way a single observer $j$ can identify the parameters $\blambda^{(j)}$. 
Nguyen et al.~\cite{Nguyen12MultiHMM}, following \cite{Vanluyten08Equal}, observed that an equivalent HMM can always be 
constructed, thereby showing that the HMM does not have a unique decomposition with permutation and scaling indeterminacy. 
Even with multiple homogeneous observers, the model is still unidentifiable,  as a consequence of failing the condition of the 
observation matrix $\bB^{(j)}$ having Kruskal's rank exceeding 1 in Theorem \ref{thm:identifiability_multi_homo}. This is in line
with the observation for homogeneous observers in \cite{Nguyen12PPHMM,Nguyen12MultiHMM}.

The model is, however, identifiable with multiple independent heterogeneous observers. Unlike the setting with 
homogeneous observers, there is now sufficient variability for identifiability, even though each $\bB^{(j)}$ may have a 
Kruskal rank of 1, as long as Theorem \ref{thm:identifiability_multi_hetero} is satisfied. By Corollary
\ref{cor:identifiability_multi_hetero}, at least two observers are sufficient for the HMM to be identified,
since 
\ben
\krank(\bA) + \krank(\bB^{(1)}) + \krank(\bB^{(2)}) \ge 7+2 = 9. 
\een
Thus, our framework provides an alternative explanation as to why it is possible to identify the HMM in the heterogeneous 
setting compared to the homogeneous setting for the network anomaly detection problem, and why at least two observers are 
required to identify the HMM, despite the observation matrices $\bB^{(j)}$ for each observer $j$ not containing sufficient 
information for identification.
